FOBE and HOBE: First- and High-Order Bipartite Embeddings

Typical graph embeddings may not capture type-specific bipartite graph features that arise in such areas as recommender systems, data visualization, and drug discovery. Machine learning methods utilized in these applications would be better served with specialized embedding techniques. We propose two embeddings for bipartite graphs that decompose edges into sets of indirect relationships between node neighborhoods. When sampling higher-order relationships, we reinforce similarities through algebraic distance on graphs. We also introduce ensemble embeddings to combine both into a "best of both worlds" embedding. The proposed methods are evaluated on link prediction and recommendation tasks and compared with other state-of-the-art embeddings. While being all highly beneficial in applications, we demonstrate that none of the considered embeddings is clearly superior (in contrast to what is claimed in many papers), and discuss the trade offs present among them. Reproducibility: Our code, data sets, and results are all publicly available online at: http://sybrandt.com/2020/fobe_hobe.

==> sections/algorithms/algebraic_sampling.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\REQUIRE Hypergraph $H$, Samples per Object $s$, \\
         Sampled Neighbors $\gamma$, Algebraic Relaxation $a$\\
         Maximum Algebraic Distance $m$ \\
\ENSURE Lists $S_I$ and $S_O$ representing input and output samples
\FORALL{$n_i \in H_N$, $n_j \in N^s \sim \Gamma(\Gamma(n_i))$}
\label{alg:algebraic_hypergraph2vec_sampling:node_node:loop}
    \STATE{Append $\left(n_i, n_j, 0, 0, \vv{0}^\gamma, \vv{0}^\gamma\right)$ to $S_I$}\\
    \STATE{Append $\left(\textsc{AlgSim}(n_i, n_j, a, m), 0, 0\right)$ to $S_O$}
\ENDFOR
\FORALL{$e_i \in H_E$, $e_j \in E^s \sim \Gamma(\Gamma(e_i))$}
\label{alg:algebraic_hypergraph2vec_sampling:edge_edge:loop}
    \STATE{Append $\left(0, 0, e_i, e_j, \vv{0}^\gamma, \vv{0}^\gamma\right)$ to $S_I$}
    \STATE{Append $\left(0, \textsc{AlgSim}(e_i, e_j, a, m), 0\right)$ to $S_O$}
\ENDFOR
\FORALL{$n \in H_N$, $e \in E^s \sim \Gamma(\Gamma(\Gamma(n)))$ \\
    \AND $e\in H_E$, $n \in N^s \sim \Gamma(\Gamma(\Gamma(e)))$}
\label{alg:algebraic_hypergraph2vec_sampling:node_edge:loop}
    \STATE{Append $\left(n, 0, e, 0, 
                         N^{\gamma} \sim \Gamma(e), 
                         E^{\gamma} \sim \Gamma(n) \right)$
           to $S_I$}
    \STATE{$v \leftarrow \underset{e' \in \Gamma(n)}{\max}{\textsc{AlgSim}(e', e, a, m)}$}
    \label{alg:algebraic_hypergraph2vec_sampling:node_edge_similarity}
    \STATE{Append $\left(0, 0, v\right)$ to $S_O$}
\ENDFOR

\end{algorithmic}
\caption{Algebraic Hypergraph2Vec Sampling}
\label{alg:algebraic_hypergraph2vec_sampling}
\end{algorithm}

\begin{algorithm}[t]
\begin{algorithmic}[1]
\REQUIRE Same typed indices $x$ and $y$, Algebraic Relaxation $a$, \\
        Maximal Algebraic Distance $m$ 
\ENSURE Observed $x,y$ similarity $v$
\STATE{$v \leftarrow 0$}
\FORALL{$z \in \Gamma(x) \cap \Gamma(y)$}
    \STATE{$w_x \leftarrow \left(m - ||a(x) - a(z)||_2\right) / m)$}\\
    \label{alg:algebraic_same_type_sample:weight_x}
    \STATE{$w_y \leftarrow \left(m - ||a(y) - a(z)||_2\right) / m)$}\\
    \label{alg:algebraic_same_type_sample:weight_y}
    \STATE{$v \leftarrow \max(\min(w_x, w_y))$}
    \label{alg:algebraic_same_type_sample:max_min}
\ENDFOR
\RETURN $v$
\end{algorithmic}
\caption{Same-Type Algebraic Similarity (\textsc{AlgSim})}
\label{alg:algebraic_same_type_sample}
\end{algorithm}


==> sections/algorithms/boolean_sampling.tex <==
% Boolean Sampling Algorithm
\begin{algorithm}[t]
\begin{algorithmic}[1]
\REQUIRE Graph $G=(A \cup B,E)$, \\
         Samples per Node $s$, \\
         Number of Sampled Neighbors $\gamma$\\
\ENSURE Lists $S_I$ and $S_O$ representing input and output samples
\FORALL{$n_i \in N$, $n_j \in N^s \sim \Gamma(\Gamma(n_i))$}
\label{alg:boolean_hypergraph2vec_sampling:node_node}
        \STATE{Append $\left(n_i, n_j, 0, 0, \vv{0}^\gamma, \vv{0}^\gamma\right)$ to $S_I$}
        \STATE{Append $\left(1, 0, 0\right)$ to $S_O$}
\ENDFOR
\FORALL{$e_i \in E$, $e_j \in E^s \sim \Gamma(\Gamma(e_i))$}
\label{alg:boolean_hypergraph2vec_sampling:edge_edge}
        \STATE{Append $\left(0, 0, e_i, e_j, \vv{0}^\gamma, \vv{0}^\gamma\right)$ to $S_I$}
        \STATE{Append $\left(0, 1, 0\right)$ to $S_O$}
\ENDFOR
\FORALL{$n \in N$, $e \in E^s \sim \Gamma(n)$
   \AND $e\in E$, $n \in N^s \sim \Gamma(e)$}
\label{alg:boolean_hypergraph2vec_sampling:node_edge}
        \STATE{Append $\left(n, 0, e, 0, N^{\gamma} \sim \Gamma(e), E^{\gamma} \sim \Gamma(n) \right)$ to $S_I$}
        \STATE{Append $\left(0, 0, 1\right)$ to $S_O$}
\ENDFOR

\end{algorithmic}
\caption{Sampling for FOBE}
\label{alg:boolean_hypergraph2vec_sampling}
\end{algorithm}


==> sections/data/a_personalized.tex <==

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\cline{2-7}
\multicolumn{1}{c|}{}& \tilt{Amazon~~~}
& \tilt{DBLP~~~}
& \tilt{Friendster~~~}
& \tilt{Livejournal~~~}
& \tilt{MadGrades~~~}
& \tilt{YouTube~~~}
\\\hline
FOBE
	& .931 % Amazon 
	& .520 % DBLP 
	& .528 % Friendster 
	& .742 % Livejournal 
	& .733 % MadGrades 
	& .646 % YouTube 
\\\hline
HOBE
	& .819 % Amazon 
	& .554 % DBLP 
	& .667 % Friendster 
	& .834 % Livejournal 
	& .830 % MadGrades 
	& .752 % YouTube 
\\\hline
Direct Comb.
	& .692 % Amazon 
	& .703 % DBLP 
	& .522 % Friendster 
	& .692 % Livejournal 
	& .867 % MadGrades 
	& .834 % YouTube 
\\\hline
Auto-Reg. Comb.
	& .696 % Amazon 
	& {\bf.716}
	& .543 % Friendster 
	& .707 % Livejournal 
	& {\bf.881}
	& {\bf.838}
\\\hline
\hline
Deepwalk
	& .970 % Amazon 
	& .536 % DBLP 
	& .532 % Friendster 
	& .800 % Livejournal 
	& .677 % MadGrades 
	& .648 % YouTube 
\\\hline
LINE
	& .724 % Amazon 
	& .501 % DBLP 
	& .502 % Friendster 
	& .545 % Livejournal 
	& .655 % MadGrades 
	& .573 % YouTube 
\\\hline
Node2Vec
	& .831 % Amazon 
	& .502 % DBLP 
	& .505 % Friendster 
	& .548 % Livejournal 
	& .629 % MadGrades 
	& .505 % YouTube 
\\\hline
BiNE
	& .517 % Amazon 
	& .672 % DBLP 
	& .501 % Friendster 
	& .535 % Livejournal 
	& .501 % MadGrades 
	& .534 % YouTube 
\\\hline
Metapath2Vec++
	& {\bf.991}
	& .584 % DBLP 
	& {\bf.757}
	& {\bf.964}
	& .769 % MadGrades 
	& .699 % YouTube 
\\\hline

\end{tabular}
\caption{\label{}}
\end{table}
\setlength\extrarowheight{0pt}


==> sections/data/b_personalized.tex <==

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\cline{2-7}
\multicolumn{1}{c|}{}& \tilt{Amazon~~~}
& \tilt{DBLP~~~}
& \tilt{Friendster~~~}
& \tilt{Livejournal~~~}
& \tilt{MadGrades~~~}
& \tilt{YouTube~~~}
\\\hline
FOBE
	& .983 % Amazon 
	& .554 % DBLP 
	& .677 % Friendster 
	& .919 % Livejournal 
	& .760 % MadGrades 
	& .604 % YouTube 
\\\hline
HOBE
	& .902 % Amazon 
	& .605 % DBLP 
	& .794 % Friendster 
	& .959 % Livejournal 
	& .878 % MadGrades 
	& .788 % YouTube 
\\\hline
Direct Comb.
	& .772 % Amazon 
	& .532 % DBLP 
	& .753 % Friendster 
	& .905 % Livejournal 
	& .885 % MadGrades 
	& .776 % YouTube 
\\\hline
Auto-Reg. Comb.
	& .782 % Amazon 
	& .525 % DBLP 
	& .784 % Friendster 
	& .941 % Livejournal 
	& {\bf.892}
	& .771 % YouTube 
\\\hline
\hline
Deepwalk
	& .980 % Amazon 
	& .523 % DBLP 
	& .641 % Friendster 
	& .896 % Livejournal 
	& .678 % MadGrades 
	& .612 % YouTube 
\\\hline
LINE
	& .926 % Amazon 
	& .579 % DBLP 
	& .860 % Friendster 
	& .970 % Livejournal 
	& .771 % MadGrades 
	& .693 % YouTube 
\\\hline
Node2Vec
	& .960 % Amazon 
	& {\bf.738}
	& .858 % Friendster 
	& .965 % Livejournal 
	& .772 % MadGrades 
	& {\bf.790}
\\\hline
BiNE
	& .514 % Amazon 
	& .500 % DBLP 
	& .500 % Friendster 
	& .500 % Livejournal 
	& .500 % MadGrades 
	& .518 % YouTube 
\\\hline
Metapath2Vec++
	& {\bf.991}
	& .587 % DBLP 
	& {\bf.869}
	& {\bf.974}
	& .770 % MadGrades 
	& .661 % YouTube 
\\\hline

\end{tabular}
\caption{\label{}}
\end{table}
\setlength\extrarowheight{0pt}


==> sections/data/data_sources.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|l|c|rr|rr|r|r|}
    \hline
     &  
     &\multicolumn{2}{c|}{$\Gamma(\alpha_i)$}
     &\multicolumn{2}{c|}{$\Gamma(\beta_j)$}
    & &\\
    Graph &
     $\nicefrac{|A|}{|B|}$
     &\multicolumn{2}{c|}{md \hfill max}
     &\multicolumn{2}{c|}{md \hfill max}
     &SR
     &LCP
    \\
    \hline
    Amazon
      &$\nicefrac{16,716}{5,000}$
      &3&49
      &8&328
      &75.8
      &1.6
    \\
    DBLP
      &$\nicefrac{93,432}{5,000}$
      &1&12
      &8&7,556
      &174.7
      &81.7
    \\
    Friendster
      &$\nicefrac{220,015}{5,000}$
      &1&26
      &133&1,612
      &80.3
      &58.3
    \\
    Livejournal
      &$\nicefrac{84,438}{5,000}$
      &1&20
      &16&1,441
      &100.9
      &27.0
    \\
    MadGrades
      &$\nicefrac{11,951}{6,462}$
      &3&39
      &4&393
      &57.3
      &99.7
    \\
    YouTube
      &$\nicefrac{39,841}{5,000}$
      &1&54
      &4&2,217
      &113.3
      &80.6
    \\
    \hline
    \end{tabular}
    \caption{\label{tab:data_sources}
    {\bf Graph Summary.} We report the median (md) and max degree for each node set, as well as the Spectral Radius (SR) and the percentage of the largest connected component (LCP).
    }
\end{table*}





==> sections/data/unified.tex <==

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\cline{2-7}
\multicolumn{1}{c|}{}& \tilt{Amazon~~~}
& \tilt{DBLP~~~}
& \tilt{Friendster~~~}
& \tilt{Livejournal~~~}
& \tilt{MadGrades~~~}
& \tilt{YouTube~~~}
\\\hline
FOBE
	& .962 % Amazon 
	& .713 % DBLP 
	& .756 % Friendster 
	& .914 % Livejournal 
	& .908 % MadGrades 
	& .846 % YouTube 
\\\hline
HOBE
	& .926 % Amazon 
	& .788 % DBLP 
	& .829 % Friendster 
	& .925 % Livejournal 
	& .913 % MadGrades 
	& .837 % YouTube 
\\\hline
Direct Comb.
	& .877 % Amazon 
	& .746 % DBLP 
	& .639 % Friendster 
	& .866 % Livejournal 
	& .910 % MadGrades 
	& .847 % YouTube 
\\\hline
Auto-Reg. Comb.
	& .876 % Amazon 
	& .754 % DBLP 
	& .684 % Friendster 
	& .883 % Livejournal 
	& {\bf.916}
	& {\bf.869}
\\\hline
\hline
Deepwalk
	& .987 % Amazon 
	& .754 % DBLP 
	& .731 % Friendster 
	& .966 % Livejournal 
	& .863 % MadGrades 
	& .832 % YouTube 
\\\hline
LINE
	& .990 % Amazon 
	& .736 % DBLP 
	& .871 % Friendster 
	& .983 % Livejournal 
	& .904 % MadGrades 
	& .854 % YouTube 
\\\hline
Node2Vec
	& .951 % Amazon 
	& .749 % DBLP 
	& .799 % Friendster 
	& .957 % Livejournal 
	& .883 % MadGrades 
	& .852 % YouTube 
\\\hline
BiNE
	& .644 % Amazon 
	& {\bf.797}
	& .608 % Friendster 
	& .651 % Livejournal 
	& .628 % MadGrades 
	& .764 % YouTube 
\\\hline
Metapath2Vec++
	& {\bf.991}
	& .791 % DBLP 
	& {\bf.885}
	& {\bf.986}
	& .906 % MadGrades 
	& .852 % YouTube 
\\\hline

\end{tabular}
\caption{\label{}}
\end{table}
\setlength\extrarowheight{0pt}

